Two stage cluster for resource optimization with Apache Mesos

As resource estimation for jobs is difficult, users often overestimate their requirements. Both commercial clouds and academic campus clusters suffer from low resource utilization and long wait times as the resource estimates for jobs, provided by users, is inaccurate. We present an approach to statistically estimate the actual resource requirement of a job in a Little cluster before the run in a Big cluster. The initial estimation on the little cluster gives us a view of how much actual resources a job requires. This initial estimate allows us to accurately allocate resources for the pending jobs in the queue and thereby improve throughput and resource utilization. In our experiments, we determined resource utilization estimates with an average accuracy of 90% for memory and 94% for CPU, while we make better utilization of memory by an average of 22% and CPU by 53%, compared to the default job submission methods on Apache Aurora and Apache Mesos.

==> old_intro.tex <==

\if0

\textcolor{red}{ Running jobs in clustered environment always have a possibility that the computational resources are not being used in an optimized way. Each job is different in term of required resources and the order in which jobs appear in a job queue always has an impact on how well the resources can be utilized. Our initial research has shown that user submits jobs with resource requirements which are more than required and cluster runs those jobs with blocking this extra computational resources. Our plan is to figure out a way and prove that if we can cut down these extra assigned resources without impacting the job's execution requirement in an optimal way then we can fit more jobs running in the cluster which will directly improve the throughput of the cluster.}

\textcolor{blue}{Currently, there need for optimizing the resources for each job, this is because HPC cluster's today have huge wait times. For example, on a EC2 cluster it took about 244 seconds to acquire 64 nodes where as the same was much higher on LLNL clusters\cite{Marathe2013ACloud}. It is very evident that wait times at many large clouds is substantial. }


\textcolor{blue}{Most cloud facilities such as Amazon EC2, Microsoft Azure etc. operate at very low resource utilization, this increases the cost to operate the facilities. The usage of schedulers and cloud management tools such as Mesos still do not enable a higher resource utilization. The problem lies in the users requesting and reserving more resources than required by the applications, in most cases(70\%) 10 times the required amount of resources. There is also an issue of users under-reserving the resources. At Twitter, the cluster is managed by Mesos, which has thousands of servers have reservations reaching 80\% but the utilization is consistently below 20\%.   \cite{DelimitrouQuasar:Management}}


\textcolor{blue}{In the analysis done by Reiss et. al. using the google trace, which was collected for about 12000 machine cluster found that the the cpu allocation for high priority production jobs were at an average of 70\% whereas the cpu usage stood at an average of 25\%, similarly for memory utilization the allocations were at an average of 60-70\% but the utilization was at an average of 30-35\% for high priority production jobs.\cite{Reiss2012HeterogeneityScale}}


\textcolor{blue}{Cloud Management softwares such as Mesos \cite{Hindman2011Mesos:Center}, Omega\cite{Schwarzkopf2013Omega}, Yarn\cite{Vavilapalli2013ApacheYARN}, and Torque\cite{TORQUEManager} ask users to make resource allocation, and these allocation requests are processed by the cloud management softwares for the placement of jobs on the cluster, for example Mesos receives the resource allocation request and based on availability and resource fairness\cite{Ghodsi2011DominantTypes}, makes resource offers to frameworks such as Apache Aurora\cite{ApacheJobs.}, Marathon\cite{Marathon:DC/OS} etc. these frameworks can then accept or reject the offers.}

\textcolor{red}{ We have considered Apache Mesos based cluster to run Docker container based job's through Apache Aurora framework and gathered actual resource requirement for each job through docker swarm. In section 2, we have discussed the experimental setup and the benchmarks that we are using to measure our experimental results and in section 3, we have discussed our initial approach to run benchmarks in serial and multiple executions. Analysis of our experimental data is done in section 4 and based on the analysis we have drawn the conclusion in section 5.}

We make the following contributions in this paper.
\begin{itemize}
\item We have implemented a way to dynamically profile the incoming jobs in a cluster which helps better utilization of the cluster
\item We propose a two-staged cluster setup, the first stage to optimize the resource allocation and the second stage to run the application
\item We propose an ideal ratio for the two cluster setup for the two optimization approaches. 
\end{itemize}

\fi
	
